REST-HANDS: Rehabilitation with Egocentric Vision Using Smartglasses for Treatment of Hands after Surviving Stroke

Stroke represents the third cause of death and disability worldwide, and is recognised as a significant global health problem. A major challenge for stroke survivors is persistent hand dysfunction, which severely affects the ability to perform daily activities and the overall quality of life. In order to regain their functional hand ability, stroke survivors need rehabilitation therapy. However, traditional rehabilitation requires continuous medical support, creating dependency on an overburdened healthcare system. In this paper, we explore the use of egocentric recordings from commercially available smart glasses, specifically RayBan Stories, for remote hand rehabilitation. Our approach includes offline experiments to evaluate the potential of smart glasses for automatic exercise recognition, exercise form evaluation and repetition counting. We present REST-HANDS, the first dataset of egocentric hand exercise videos. Using state-of-the-art methods, we establish benchmarks with high accuracy rates for exercise recognition (98.55%), form evaluation (86.98%), and repetition counting (mean absolute error of 1.33). Our study demonstrates the feasibility of using egocentric video from smart glasses for remote rehabilitation, paving the way for further research.

==> tables/ex_evaluation.tex <==
\begin{table}[tb]
  \caption{Evaluation of exercises form with multi-subject tests. From the dataset, all recordings of the target subject are selected as the test subset. The methods are trained on the 90\% of the remaining data and validated on 10\% of it without networks seeing the tested subject.
  }
  \label{tab:headings}
  \centering
  \begin{tabular}{@{}lccccccccc@{}}
    \toprule
    Method & S-I & S-II & S-III & S-IV & S-V & S-VI& S-VII & S-VIII & S-IX\\
    \midrule
    SlowFast \cite{feichtenhofer2019slowfast} &\textbf{76.22} &83.84 &\textbf{82.53} &76.05 & 72.66 & 56.38 & \textbf{41.10} & 70.45 & \textbf{74.86}\\
    Swin3D \cite{liu2022video} &75.52 & \textbf{86.07} & 66.17 & 70.00 & \textbf{75.86} & \textbf{90.07} &37.86 & 62.63& 60.34\\
    MViTv2 \cite{li2022mvitv2} & 75.52 & 77.44 & 72.49 & \textbf{76.84} & 72.41 & 53.90 &38.19 & \textbf{71.72} & 69.27 \\
     
  \bottomrule
  \label{tab:ex_ev_cross_sub}
  \end{tabular}
\end{table}




==> tables/study_comparison.tex <==
\begin{table}[tb]
  \caption{}
  \label{tab:headings}
  \centering
  \begin{tabular}{@{}lccccccc@{}}
    \toprule
    Study & Year & Public& Rehab. & Egocentric & No. Partic. & No. Ex. &Tasks \\
    \midrule
    Nikishina et al.~\cite{nikishina2019application} & 2019 & ? & \checkmark & \ding{55} & 57 & 6 & ?\\
     Likitlersuang et al.~\cite{likitlersuang2019egocentric} & 2019 &?& \ding{55} &  \checkmark & 17 & - & interactions\\
    Visee et al.~\cite{visee2020effective} & 2020 &?& \ding{55} &  \checkmark & 17 & - & hand detection\\
    \midrule
    Ours & 2024 & \checkmark & \checkmark & \checkmark & 9 & 25 & Rec.; Form; Rep.\\
  \bottomrule
  \end{tabular}
\end{table}
